Unleashing the Emergent Cognitive Synergy in Large Language Models: A Task-Solving Agent through Multi-Persona Self-Collaboration

Human intelligence thrives on cognitive synergy, where collaboration among different minds yield superior outcomes compared to isolated individuals. In this work, we propose Solo Performance Prompting (SPP), which transforms a single LLM into a cognitive synergist by engaging in multi-turn self-collaboration with multiple personas. A cognitive synergist is an intelligent agent that collaboratively combines multiple minds' strengths and knowledge to enhance problem-solving in complex tasks. By dynamically identifying and simulating different personas based on task inputs, SPP unleashes the potential of cognitive synergy in LLMs. Our in-depth analysis shows that assigning multiple fine-grained personas in LLMs improves problem-solving abilities compared to using a single or fixed number of personas. We evaluate SPP on three challenging tasks: Trivia Creative Writing, Codenames Collaborative, and Logic Grid Puzzle, encompassing both knowledge-intensive and reasoning-intensive types. Unlike previous works, such as Chain-of-Thought, that solely enhance the reasoning abilities in LLMs, experimental results demonstrate that SPP effectively reduces factual hallucination, and maintains strong reasoning capabilities. Additionally, comparative experiments show that cognitive synergy only emerges in GPT-4 and does not appear in less capable models, such as GPT-3.5-turbo and Llama2-13b-chat, which draws an interesting analogy to human development. Code, data, and prompts can be found at: https://github.com/MikeWangWZHL/Solo-Performance-Prompting.git.

==> figures/impact_of_N_for_TCW_task.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{images/TCW-N-1-N-5.png}
  \caption{
  \zhenhailong{TODO} Impact of N on Trivia Creative Writing.
  }
  \label{fig:impact_N_TCW}
\end{figure}

==> figures/impact_of_question_ordering_for_TCW_task.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{images/TCW-N-5-shuffled.png}
  \caption{
  \zhenhailong{TODO} Impact of question ordering on Trivia Creative Writing.
  }
  \label{fig:impact_question_ordering}
\end{figure}

==> figures/model_comparison.tex <==
\begin{figure}[ht]
  \centering
  \includegraphics[width=0.45\textwidth]{images/model_comparision_trivia_creative_writing_avg.png}
  \vspace{-5pt}
  \caption{
    Average scores on \tasktrivia{} N=5 and N=10, comparing LLMs with various levels of capabilities. \oursabbr{} achieves superior performance only with the most powerful LLM (GPT-4), but not with GPT-3.5 and Llama2-13b. This indicates that cognitive synergy abilities only emerge in LLMs with GPT-4 level capabilities.
    \vspace{-10pt}
  }
  \label{fig:model_comparison}
\end{figure}

==> figures/persona_cloud.tex <==
\begin{figure*}[th]
  \centering
  \includegraphics[width=0.8\textwidth]{images/persona_cloud.pdf}
  \vspace{-5pt}
  \caption{
    Visualization of the \oursabbr{}-identified personas for each task. Personas identified in knowledge-intensive tasks like \tasktrivia{} are more diverse, while those in reasoning-intensive tasks like \tasklogic{} appear more homogeneous.
    % Personas identified in knowledge-intensive tasks, such as \tasktrivia{}, tend to be more diverse and specific, whereas in reasoning-intensive tasks, like \tasklogic{}, they appear more homogeneous.
    % This observation aligns with the findings in Figure~\ref{fig:spp-fixed-analysis}, which demonstrate that the benefits of dynamically identified personas are more evident in knowledge-intensive tasks.
    \vspace{-10pt}
  }
  \label{fig:persona_cloud}
\end{figure*}

==> figures/spp_vs_spp_fixed.tex <==

% %%% two column old version %%%
% \begin{figure*}[ht]
%   \centering
%   \includegraphics[width=0.6\textwidth]{images/barchart_spp_vs_spp_fixed.png}
%   \vspace{-10pt}
%   \caption{
%     Comparison between \oursabbr{} (with dynamically identified personas) and \oursfixabbr{} (with fixed personas). The results demonstrate that dynamic, fine-grained personas consistently outperform fixed, general personas.
%   }
%   \label{fig:spp-fixed-analysis}
% \end{figure*}


% %%% one colum new version %%%
% \begin{figure}[th]
%   \centering
%   \includegraphics[width=0.45\textwidth]{images/barchart_spp_vs_spp_fixed_save_space.png}
%   \vspace{-5pt}
%   \caption{
%     Comparison between \oursabbr{} (with dynamically identified personas) and \oursfixabbr{} (with fixed personas) on GPT-4. The results demonstrate that dynamic, fine-grained personas consistently outperform fixed, general personas.
%     % Another observation is that \oursfixabbr{} seems more sensitive to system messages and exhibits a unique early-termination problem (detailed in the text) that leads to unexpectedly low performance on certain tasks, such as \taskcodenames{}.
%     \vspace{-10pt}
%   }
%   \label{fig:spp-fixed-analysis}
% \end{figure}

%%% one colum new version: adding SPP-Profile and N=10 %%%
\begin{figure*}[th]
  \centering
  \includegraphics[width=0.6\textwidth]{images/barchart_spp_variants_7x4.png}
  \vspace{-5pt}
  \caption{
    \zhenhailong{TODO}
  }
  \label{fig:spp-fixed-analysis}
\end{figure*}

==> figures/teaser_figure_horizontal.tex <==
\begin{figure*}[ht]
  \centering
  \includegraphics[width=\textwidth]{images/teaser_figure_horizontal.pdf}
  \caption{
    Schematic illustration of \ours{} (\oursabbr{}) and the difference compared to previous prompting methods. 
    \oursabbr{} transforms a single LLM into a cognitive synergist that dynamically identifies personas and engages in multi-turn self-collaboration to solve various tasks effectively.
    % In \oursabbr{}, the LLM first dynamically identifies multiple useful personas and initiates a multi-turn self-collaboration before outputting the final solution. 
  }
  \label{fig:teaser_figure}
\end{figure*}

==> tables/codenames_task_table.tex <==
% % avg across w/ and w/o system message
% \begin{table*}[ht]
%     \centering  
     
%     \begin{tabular}{lcc}  
%       \toprule  
%       \textbf{Methods} & \textbf{Score (\%)} & \textbf{$\Delta$ (v.s Standard \%)} \\
%       \midrule  
%           Standard                              & 75.4   & 0.0\%\\
%           CoT                                   & 72.7   & \textcolor{textred}{-3.6\%}\\
%           \textbf{SPP-Profile (ours)}           & 76.7   & \textcolor{textgreen}{+1.7\%}\\
%           \textbf{SPP (ours)}                   & \textbf{79.0}   & \textcolor{textgreen}{\textbf{+4.8\%}}\\
%       \bottomrule  
%     \end{tabular}

%     \caption{\taskcodenames{} main results. $\Delta$ indicates the relative gain/loss compared with Standard Prompting (first row).}
%   \label{tab:codenames_task_results}  
% \end{table*}  




% avg across w/ and w/o system message
\begin{table}[th]
    \small
    \centering  
    \begin{tabular}{lcc}  
      \toprule  
      \textbf{Methods} & \textbf{Score (\%)} & \textbf{$\Delta$ (\%)} \\
      \midrule  
          Standard                              & 75.4   & 0.0\%\\
          CoT                                   & 72.7   & \textcolor{textred}{-3.6\%}\\
          \textbf{SPP-Profile (ours)}           & 76.7   & \textcolor{textgreen}{+1.7\%}\\
          \textbf{SPP (ours)}                   & \textbf{79.0}   & \textcolor{textgreen}{\textbf{+4.8\%}}\\
      \bottomrule  
    \end{tabular}

    \caption{\taskcodenames{} GPT-4 results. $\Delta$ indicates the relative gain/loss compared with Standard Prompting (first row).
    \vspace{-10pt}
    }
  \label{tab:codenames_task_results}  
\end{table}  




==> tables/logic_task_table.tex <==
\begin{table}[th]
    \small
    \centering 
    \begin{tabular}{lcc}  
      \toprule  
      \textbf{Methods} & \textbf{Score (\%)} & \textbf{$\Delta$ (\%)} \\
      \midrule  
          Standard                              &   57.7  & 0.0\%  \\
          CoT                                   &   65.8  & \textcolor{textgreen}{+14.1\%} \\
          \textbf{SPP-Profile (ours)}           &   64.8  & \textcolor{textgreen}{+12.4\%} \\
          \textbf{SPP (ours)}                   &   \textbf{68.3}  & \textcolor{textgreen}{\textbf{+18.5\%}} \\
      \bottomrule  
    \end{tabular}
    \caption{\tasklogic{} GPT-4 results. $\Delta$ indicates the relative gain/loss compared with Standard Prompting (first row).}
    
  \label{tab:logic_task_results}  
\end{table}  

% \begin{table*}[ht]
%     \centering  
     
%     \begin{tabular}{lcc}  
%       \toprule  
%       \textbf{Methods} & \textbf{Score (\%)} & \textbf{$\Delta$ (v.s Standard \%)} \\
%       \midrule  
%           Standard                              &   57.7  & 0.0\%  \\
%           CoT                                   &   65.8  & \textcolor{textgreen}{+14.1\%} \\
%           \textbf{SPP-Profile (ours)}           &   64.8  & \textcolor{textgreen}{+12.4\%} \\
%           \textbf{SPP (ours)}                   &   \textbf{68.3}  & \textcolor{textgreen}{\textbf{+18.5\%}} \\
%       \bottomrule  
%     \end{tabular}
%     \caption{\tasklogic{} Main Results. $\Delta$ indicates the relative gain/loss compared with Standard Prompting (first row).}
    
%   \label{tab:logic_task_results}  
% \end{table*}  

==> tables/trivia_task_table.tex <==
\begin{table*}[th]
    \small
    \centering
    \begin{tabular}{l | cc | cc}  
      \toprule  
      \multirow{2}{*}{\textbf{Methods}}
      & \multicolumn{2}{c|}{\textbf{N (\# trivia questions) = 5 }}
      & \multicolumn{2}{c}{\textbf{N (\# trivia questions ) = 10}}\\
      & \textbf{Score (\%)} & \textbf{$\Delta$ (\%)} & \textbf{Score (\%)} & \textbf{$\Delta$ (\%)} \\
      \midrule  
          Standard                              & 74.6            & 0.0\%                                       & 77.0            & 0.0\%                                       \\  
          CoT                                   & 67.1            & \textcolor{textred}{-10.0\%}                & 68.5            & \textcolor{textred}{-11.1\%}                \\  
          \textbf{SPP-Profile (ours)}                    & 79.1            & \textcolor{textgreen}{+5.9\%}               & 83.0            & \textcolor{textgreen}{+7.8\%}               \\  
          \textbf{SPP (ours) }                           & \textbf{79.9}   & \textcolor{textgreen}{\textbf{+7.1\%}}      & \textbf{84.7}   & \textcolor{textgreen}{\textbf{+10.0\%}}      \\  
      \bottomrule  
    \end{tabular}
  \caption{\tasktrivia{} GPT-4 results. $\Delta$ indicates the relative gain/loss compared with Standard Prompting (first row). \vspace{-10pt}} 

  \label{tab:trivia_task_results}  
\end{table*}  


